Learning to Reason via Program Generation, Emulation, and Search

Program synthesis with language models (LMs) has unlocked a large set of reasoning abilities; code-tuned LMs have proven adept at generating programs that solve a wide variety of algorithmic symbolic manipulation tasks (e.g. word concatenation). However, not all reasoning tasks are easily expressible as code, e.g. tasks involving commonsense reasoning, moral decision-making, and sarcasm understanding. Our goal is to extend an LM's program synthesis skills to such tasks and evaluate the results via pseudo-programs, namely Python programs where some leaf function calls are left undefined. To that end, we propose, Code Generation and Emulated EXecution (CoGEX). CoGEX works by (1) training LMs to generate pseudo-programs, (2) teaching them to emulate their generated program's execution, including those leaf functions, allowing the LM's knowledge to fill in the execution gaps; and (3) using them to search over many programs to find an optimal one. To adapt the CoGEX model to a new task, we introduce a method for performing program search to find a single program whose pseudo-execution yields optimal performance when applied to all the instances of a given dataset. We show that our approach yields large improvements compared to standard in-context learning approaches on a battery of tasks, both algorithmic and soft reasoning. This result thus demonstrates that code synthesis can be applied to a much broader class of problems than previously considered. Our released dataset, fine-tuned models, and implementation can be found at \url{https://github.com/nweir127/CoGEX}.

==> old/ablations.tex <==
\begin{table}[ht!]
    \centering
    \begin{tabular}{lrrrr}
\toprule
 & \multicolumn{2}{c}{llama-2-7b} & \multicolumn{2}{c}{llama-2-13b} \\
 & (+/-) & plan (+/-) & (+/-) & plan (+/-) \\
\midrule
\textbf{cola} & 12.8 & -0.1 & 9.3 & -1.7 \\
\textbf{emotion} & 11.3 & -0.9 & 1.0 & 1.7 \\
\textbf{sst} & 45.8 & 2.3 & 39.6 & 2.3 \\
\textbf{coin flip} & 15.2 & 9.5 & 21.9 & 9.5 \\
\textbf{tracking shuffled objects} & 0.4 & -4.7 & 1.2 & 1.3 \\
\textbf{sum} & 2.2 & 45.8 & 3.5 & 29.6 \\
\textbf{svamp} & 0.7 & 21.7 & 2.7 & 12.0 \\
\textbf{commonsense qa} & 28.4 & 5.6 & 9.1 & 6.5 \\
\textbf{social i qa} & 26.9 & 9.0 & 23.2 & -0.2 \\
\bottomrule
\end{tabular}

    \caption{delta against direct answering (+/-; decoding a separate program for each input instance) and against search over text plan (plan (+/-); training a model to generate only the NL plan steps before returning the output dictionary, then running \search{} to find an optimal task-specific plan.)
    \todo{nate change to plot}
    }
    \label{tab:my_label}
\end{table}

==> sections/1_introduction-old-v1.tex <==
\section{Introduction}


\begin{comment}
{\color{red}

from peter:
 
LMs have proven deft at answering algorithmic questions via code synthesis,
e.g., answering "What is the concatenation of the 3rd letter of every word in <sentence>?" by generating and executing Python code.
But what about tasks that require commonsense or judgemental steps (e.g., ``determine the most likely location of <object>''),
not easily formulated as code?
Our goal is to extend a LM's program synthesis skills to such tasks, and evaluate the results.
Our approach is to first have the LM generate {\it partial programs}, where “soft” leaf function
calls (e.g., likely
$\_$location(object)) are left undefined, and then second use the LM to {\it simulate}
execution of the program, including the likely results of such function calls, to
produce both intermediate results and a final answer.
We use a search method blah blah
Our results show blah blah
This is significant, as it shows how an integration of ideas from partial programming, simulated code execution, and
search can allow programmatic-based solutions to be applied to a much broader class of problems than previously considered.


}
\end{comment}


%Instruction tuning language models (LMs) is typically done by training models to follow user instructions purely formatted  
Reasoning with language models (LMs) is typically done in natural language (NL) \citep{wei22,zhang2023instruction}, where the model input, output, and 
elicited intermediate reasoning steps from are in NL.
However, NL has its own limitations when, for example, the given task requires generating, manipulating, or tracking structures such as lists or nested objects.
% or performing algorithmic reasoning. 
Recent work has explored the possibility of training LMs to reason over code, relying on the intuition that code may be more effective than NL for different reasoning scenarios \citep{chen2022program,gao-etal-2023-pal}. Additionally, utilizing code interpreters can bring extra benefit since the LM only needs to generate a program that achieves the task \citep{li2023chain}.
While successful, such works are mainly limited to tasks conducive to a programmatic paradigm:
symbolic manipulation, algorithmic reasoning, and math, i.e., tasks for which a compilable program might exist. This is not the case, however, for ``softer'' reasoning tasks such as commonsense and social reasoning tasks, which can not be purely solved in code \citep{zhang2023exploring}. 


%\llq{should we mention the motivation of using LM as the code emulator? e.g. these approaches mostly rely on using python interpreter. However, for many general tasks, it is less obvious how to write and execute a program?}
%\nw{agreed, we should lean more on that}
Our work investigates whether it is possible to sidestep actual code interpreters and use LMs to emulate code interpretation. We inquire:
Can LMs reason by generating and emulating code? The code generated could describe well-defined, precise reasoning steps such as in the case of math or algorithmic tasks, but could also delineate more fuzzy forms of reasoning, such as commonsense.
%tasks that require flexibly applying input-specific pieces of world knowledge?
This works aims to explore whether such soft reasoning tasks can be performed if we they are formulated in code that is pseudo-executed by the LM. 
%and equal or exceed performance by LMs that use purely NL?

\begin{figure}[t!]
    \centering
        \includegraphics[width=.9\textwidth]{figures/instrucode_flowchart_colored.pdf}
    %     \quad 
    % \includegraphics[width=0.55\linewidth]{figures/alpaca-code.pdf}
    \caption{Example from the \dataset{} dataset automatically converted from an Alpaca~\citep{taori2023alpaca} instance via LLM prompting. We train the model to receive the instruction and input and generate the Python program, function call, and output dictionary containing the answer. 
    % \mk{should we show intermediate outputs from each stage?} \nw{I think it's relatively straightforward. step 2 is in pink, i can shade the box on the left too\dots} \mk{shading works-- consider shading step 1 and 3 as well.}
    }
    \label{fig:data-construction}
\end{figure}

To explore these questions, we propose a novel framework:
% As opposed to training LMs to take and follow instruction in natural language, 
% our work explores a novel paradigm: 
training models to follow NL instructions by converting  them to code and \textit{emulating} code execution. Our paradigm, dubbed \method, 
% trains a model to perform instruction following by flexibly generating and executing its own program in well-formed Python syntax.
% Our method 
alters the inference process to \textbf{(i)} generate a Python function given an arbitrary instruction and optional input,  \textbf{(ii)}
generate a call to that function, and \textbf{(iii)} produce the result of simulating its execution. 
Unlike other work~\citep{zhang-etal-2023-natural,li2023chain}, we do not use a Python interpreter to execute any code; rather, the model executes it implicitly.
%\llq{should we mention \citet{chae2024language, li2023chain}, i guess the main difference is they are still mostly focusing on symbolic tasks but we consider general tasks?}
This allows for the model's program to frequently invoke \textit{deliberately underspecified functions}
that allow the model to flexibly reason about instances without the potential constraints of formal programmatic definition.
We train the model to not only produce an answer to an instruction, but also the results of intermediate reasoning steps that reflect a high-level plan for how to respond. 
This gives us an improved level of behavioral interpretability and systematicity.
\method moreover suggests a way to leverage the flexible ad-hoc reasoning of LLMs as subroutines while encouraging programmatic reason via the top-level program.
We train \method models by adapting the recent Alpaca instruction tuning dataset~\citep{taori2023alpaca} into a set of analogous Pythonic examples. 
We propose a pipeline that uses prompts to an LLM (e.g. GPT-4) to perform the dataset conversion automatically and then use the resulting \dataset dataset to fine-tune smaller (7B and 13B) LLMs to answer instructions by reasoning over code.

When given an LLM and $N$ training examples currently, NLP practicioners use the examples for in-context learning.
Training a model to generate then apply a function given input instructions raises an intriguing new alternative to this {learning} paradigm:
finding a program that best solves a new task, then applying the program to new instances of the task by letting the \method model generate new calls to it.
Inspired by work on hard prompt tuning~\citep{wen-etal-2024-hard} and example selection for in-context learning~\citep{gupta-etal-2023-coverage}, 
we introduce a search procedure that uses the frozen
\method{} model to try out many programs on a set of training examples and identify which single program is most generalizable across the dataset. We call the procedure \searchlong{}, which performs no parameter updates and requires saving nothing more than the single \method{} checkpoint and separate task-specific programs for each new dataset to be handled. 
% \ow{We don't require the user to give these programs right?} \nw{right, the model finds the program automatically}

We evaluate over a diverse suite of reasoning tasks, including commonsense QA, text classification, and math datasets. 
We find that \search{}  leads the \method{} model to substantially outperform the comparable natural language-based LLM using the same original checkpoint and the same set of training examples available for in-context learning, even in the few-shot regime.
\search{} thus gives us one way to fit a model to a new dataset without having to perform any gradient descent or parameter updates beyond finding and saving a task-specific program. 
% This makes \search a particularly helpful method, even when LM providers do not wish to release model weights.
% We show that \search{} provides these benefits over .
While existing work on code-based reasoning has either primarily considered symbolic manipulation tasks~\citep{gao-etal-2023-pal} or required additional entailment classifiers~\citep{zhang-etal-2023-natural}, ours requires only the LM checkpoint and applies broadly to general NLP and reasoning tasks.
% and a systematically searched-for, task-specific program.




Our contributions are thus:
\begin{enumerate}
\item A novel instruction tuning paradigm, \method{}, that trains language models to 
generate and emulate the execution of Python code in order to follow an instruction or perform a task.
\item A open-source code-based version of the 52K Alpaca instruction following demonstrations for fine-tuning \method{} models.
\item A novel tuning paradigm, \search{}, that casts learning as a code search using a training set. This shows to improve a 7B and 13B-parameter \method{} models on a wide array of tasks, including not only code-friendly tasks like math and algorithmic symbolic manipulation, but also a wide array of other kinds of tasks that require reasoning over natural language text and world knowledge, compared to their standard instruction tuning and few-shot setups. 
% We show how code-based reasoning models can be effectively applied to not only to code-friendly tasks like math and algorithmic symbolic manipulation, but also a wide array of other kinds of tasks that require reasoning over natural language text and world knowledge.

\end{enumerate}

Our released \dataset{} dataset, fine-tuned models, and code for the \search{} program search algorithm can be found at 
<anonymized>.
% \url{https://www.booking.yeah}



==> tables/qa_main.tex <==
\begin{table}[ht]
\small
\setlength{\tabcolsep}{3pt} 
    \centering
    

\scalebox{0.9}{
% \begin{tabular}{p{2.2cm}lrrrrrrrrr|c}
\begin{tabular}{p{2.2cm}lcccccccccc|c}
\toprule
& & & \multicolumn{3}{c}{\textbf{Classification}} & \multicolumn{2}{c}{\textbf{Symbolic}} & \multicolumn{2}{c}{\textbf{Math}} & \multicolumn{2}{c}{\textbf{Commonsense}} & 
%  \multicolumn{1}{c}{\textbf{Average}} 
\\
\cmidrule(lr){4-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} 
% \cmidrule(lr){12-12}
& &  $N_{\text{train}}$ & CoLA & Emotn & SST & Coin & WSort & Sum & SVAMP & CSQA & SIQA & \textbf{Avg} \\
\midrule
Alpaca 7B & 0-shot & 0 & 70.6 & 53.4 & 87.3 & 49.5 & 40.0 & 21.6 & 25.7 & 46.8 & 54.1 & 49.9 \\
\midrule
Llama-2 7B & 2-S BM25 & 1000 & 57.5 & 55.2 & 82.1 & 32.4 & 45.5 & 35.2 & 34.7 & 45.7 & 46.0 & 48.3 \\
\midrule
\multirow[t]{3}{2.2cm}{\textbf{\method} Llama-2 7B} & \search{} $k=1$ & 10 &  \up 75.0 & \dn 52.2 & \up 86.9 & \up 50.8 & \dn 40.6 & \up 61.3 & \dn 33.3 & \dn 42.3 & \up 50.1 &   56.7 \\
 & \search{} ${k=1}$ & 1000 & \up 78.5 & \up 56.2 & \up 91.2 & \up 60.0 & \dn 39.5 & \up 62.8 & \up 41.3 & \up 52.7 &\up  57.7 & 60.0 \\
 & \search{} ${k=3}$ & 1000 & \up 79.2 & \up 56.0 & \up 90.9 & 61.9 \up & \dn 40.8 & \up 63.6 & \up 42.7 & 52.4 \up & \up 59.3 & \textbf{60.8} \\
\midrule 
CodeLlama 7B & 2-S BM25 & 1000 & 70.9 & 56.2 & 90.9 & 31.4 & 38.7 & 33.6 & 35.0 & 46.5 & 55.8 & 51.0 \\
\midrule
\multirow[t]{3}{2.2cm}{\textbf{\method} CodeLlama 7B} & \search{} $k=1$ & 10 &  \up 77.0 & \dn 54.6 & \dn 76.2 & \up 52.6 & \up  44.5 & \up  54.1 & \dn 32.6 & \up 51.2 & \dn 51.1 & 54.9 \\
& \search{} ${k=1}$ & 1000 & \up 76.7 & \up 58.0 & \dn 87.5 & \up 67.6 & \up 44.7 & \up 57.0 & \up 36.7 & \up  52.9 & \dn 55.1 & 59.6 \\
& \search{} ${k=3}$ & 1000 & 77.9 \up & 56.8 \up & 89.7 \dn & 72.4 \up & 45.3 \up & 57.4 \up & 40.0 \up & 56.0 \up & 55.1 \dn & \textbf{61.2 }\\
\midrule \midrule
Alpaca 13B & 0-shot & 0 & 74.6 & 53.0 & 86.0 & 63.8 & 50.3 & 44.5 & 37.3 & 62.2 & 63.4 & 59.5 \\
\midrule
\multirow[t]{2}{2.2cm}{Llama-2 13B} & 2-S BM25 & 1000 & 78.9 & 54.0 & \textbf{92.4} & 48.6 & 50.0 & 38.7 & 46.0 & 63.4 & 62.8 & 59.4 \\
% & \textbf{Fine-tuning} & 1000 & 74.2 & 82.5 & 94.7 & 60.0 & 55.3 & 76.9 & 54.0 & 74.2 & 68.4 & 71.1 \\
\midrule
\multirow[t]{3}{2.2cm}{\textbf{\method} Llama-2 13B} & \search{} $k=1$ & 10 & \up 80.9 & \up 55.1 & \dn 88.9 & \dn 58.0 & \up 51.3 & \up 61.3 & \dn 42.8 & \dn 59.2 & \dn 57.6 & 61.7 \\
& \search{} ${k=1}$ & 1000 & \up 81.0 & \up  56.4 & \dn 92.1 & \up 65.7 & \up  50.8 & \up  64.0 & \up 48.3 & \same 63.4 &  \up 64.6 & 65.1 \\
& \search{} ${k=3}$ & 1000 & \up \textbf{81.0} & \up 56.6 & \dn 92.1 & \up 69.5 & \up \textbf{51.6} & \up 63.9 & \up \textbf{50.3} & \up \textbf{64.0} & \up \textbf{65.5} & \textbf{66.1} \\
\midrule
CodeLlama 13B & 2-S BM25 & 1000 & 74.3 & \textbf{60.3} & 91.6 & 74.3 & 50.3 & 59.2 & 43.3 & 51.8 & 57.8 & 62.6 \\
\midrule
\multirow[t]{3}{2.2cm}{\textbf{\method} CodeLlama 13B} & \search{} $k=1$ & 10 &  \up 80.4 & \dn 55.8 & \dn 89.7 & \dn 53.5 & \dn 49.4 & \up  71.4 & \up  43.9 & \dn 52.2 & \dn 55.5 & 61.3 \\
\multirow[t]{3}{2.2cm}{}
 & \search{} ${k=1}$ & 1000 & \up 80.4 & \dn 56.1 & \dn 90.4 & \up  86.7 & \dn 48.4 & \up  73.7 & \up  46.7 & \dn 58.0 & \dn 60.0 & \textbf{66.7} \\
 & \search{} ${k=3}$ & 1000 & \up 80.5 & \dn 56.4 & \dn 91.2 & \up 81.9 & \dn 49.2 & \up \textbf{74.2} & \up 47.3 & \dn 57.2 & \dn 60.8 & 66.5 \\
\bottomrule
\end{tabular}
}

\caption{Benchmark results by fine-tuned \method{} models optimized for each dataset using the \search{} method, compared to the corresponding off-the-shelf checkpoint Llama-2/CodeLlama models 
 performing 2-shot reasoning using a BM25 retrieval index of 1000 exemplars. Results also compared to the same-sized Alpaca model fine-tuned from Llama-2.
 Colored cells indicate changes (\greentext{gains}, \redtext{losses}, or the \greytext{same}) relative to the best-performing non-\method{} baseline (between Alpaca and 2-shot with the same base checkpoint).
% \todo{add column for avg.}
% \nw{need a new way to distinguish "10-shot" from the BM25 row, which is using all 1000 examples via dynamic retrieval} {why are some rows not highlighted?}
}

    \label{tab:main_results}
\end{table}
